Precoding for Satellite Communications: Why, How and What next?

Precoding has stood out as a promising multi-user transmission technique to meet the emerging throughput demand of satellite communication systems while awaiting the technological maturity for exploiting higher bands. Precoding enables the reduction of interference among co-channel beams through spatial processing while promoting aggressive frequency reuse and improving spectral efficiency. Satellite systems offer multitude of system and service configurations, resulting in different precoder design methodologies. This article explores the motivation for the introduction of precoding, offers an insight to their theoretical development in a diverse scenarios and presents some avenues for future development.

==> Part2.tex <==
\subsection{Architecture and Communication Peculiarities}

This is the case of precoding techniques that allow a high frequency reuse factor among different beams. With the aid of precoding, a satellite UT can obtain a sufficiently large signal to interference and noise ratio (SINR) even though the carrier bandwidth is reused by adjacent beams. In order to maintain a certain SINR value, the precoder mitigates the interference that can affect the  satellite UT.

 
\begin{enumerate}

\item \emph{The co-channel interference power does not decrease as the number of beams increases.} The favorable propagation in massive MIMO mentioned in \cite{massive1} does not occur in multibeam satellite systems. That is, in a scattered terrestrial channel environment, the off-diagonal elements of the channel covariance matrix tend to zero as the number of antennas grows, leading to an ideal interference-free scenario. On the contrary, due to the low scatter in the satellite channel, there is always strong co-channel interference among beams independent of the dimension of the multibeam satellite system. 

\item \emph{There is no pilot contamination.} Massive MIMO in multicell scenarios entails difficulties in the channel estimation operation as users located in adjacent cells might inject interference into the estimation process. In the multibeam satellite case, this does not occur since the number of adjacent beams in a given area is limited. Also, the pilot signals of adjacent beams are orthogonal, and the satellite channel is, in general, non-frequency-selective and preserves the orthogonality at the UT.

\item \emph{Multibeam satellite systems can naturally perform multicast transmission.} Due to the large coverage area of each satellite beam, which is in the order of few hundred kms, most of the satellite communication standards assume that a transmitted codeword would contain information from more than one UT, leading to a channel coding gain with respect to the case where short individual codewords are used.

\end{enumerate}


\subsection{Precoding Techniques}

Let us consider a multibeam satellite system in which the satellite is equipped with an array-fed reflector antenna with a total number of feeds equal to $N$. These feed signals are combined to generate a beam radiation pattern composed of $K$ beams, which is considered fixed. For each frame, we assume that a total number of $N_u$ users are simultaneously served per beam (i.e., the total number of served users by the satellite is $KN_u$). Considering that all beams radiate in the same frequency band (i.e., $f_{r}=1$), the instantaneous received signal at the $i$-th user terminal of each beam is given by
\begin{equation}\label{sys}
\mathbf{y}^{[i]} = \mathbf{H}^{[i]} \mathbf{x} + \mathbf{n}^{[i]}, \quad  i = 1, \ldots , N_u,
\end{equation}
where vector $\mathbf{y}^{[i]} \in \mathbb{C}^{K \times 1}$ is the vector containing the received signals of the $i$-th UT (i.e., the value $\left[\mathbf{y}^{[i]} \right]_k$ refers to the received signal of the $i$-th UT at the $k$-th beam), whereas vector $\mathbf{n}^{[i]} \in \mathbb{C}^{K \times 1}$ contains the noise terms of each $i$-th UT. The entries of $\mathbf{n}^{[i]}$ are assumed  to be independent and Gaussian distributed with zero mean and unit variance (i.e., $E\left[\mathbf{n}^{[i]} {\mathbf{n}^{[i]}}^H \right] = \mathbf{I}_{K} \quad i = 1, \ldots , N_u$). Finally, vector $\mathbf{x} \in \mathbb{C}^{K \times 1}$ contains all the transmitted signals.

The channel matrix can be described as follows:
\begin{equation}\label{cc}
\mathbf{H}^{[i]} = \mathbf{F}^{[i]} \circ \overline{\mathbf{H}}^{[i]}, \quad  i = 1, \ldots , N_u,
\end{equation}
where the $(k,n)$-th entry of matrix $\overline{\mathbf{H}}^{[i]}  \in  \mathbb{R}^{K \times N}$ is 

\begin{equation}\label{ccana}
\left[\overline{\mathbf{H}}^{[i]}  \right]_{k,n} = \frac{G_Ra_{kn}^{[i]} e^{j\psi_{k,n}^{[i]}}}{4 \pi \frac{d_{k}^{[i]}}{\lambda} \sqrt{K_BT_RB_W}}\;k=1, \ldots , K; n=1, \ldots , N; i=1, \ldots , N_u.
\end{equation}

$d_{k}^{[i]}$ is the distance between the $i$-th UT at the $k$-th beam and the satellite. $\lambda$ is the carrier wavelength, $K_B$ is the Boltzmann constant, $B_W$ is the carrier bandwidth, $G_R^2$ is the UT receive antenna gain, and $T_R$ is the receiver noise temperature. The term $a_{kn}^{[i]}$ refers to the gain from the $n$-th feed to the $i$-th user at the $k$-th beam. The time varying phase due to beam radiation pattern and the radio wave propagation is represented by $\psi_{k,n}^{[i]}$. Note that we have considered that the feeder link is ideal and its impact is limited to a scaling factor. 

Furthermore, matrix $\mathbf{F}^{[i]} \in \mathbb{C}^{K \times N}$ represents the atmospheric fading such that $\left[\overline{\mathbf{F}}^{[i]}  \right]_{k,n} = \mu_k^{[i]}e^{j\theta_k^{[i]}}$, where notably  each fading coefficient is independent of the transmission feed. That is, the UT experiences a fading value that equally impacts all feed signals. There is no multipath and a strong line-of-sight is present in frequencies above 10 GHz (i.e., above the Ku band), whenever there is no blockage.

In order to mitigate the co-channel interference due to the high frequency reuse factor, precoding is performed; therefore, the transmitted signal vector per beam is given by $\mathbf{x} = \mathbf{W}\mathbf{s},$ where $\mathbf{s} \in \mathbb{C}^{K \times 1}$ is the vector that contains the transmitted symbols per UT, which we assume are uncorrelated and unit normed $\left(E\left[\mathbf{s}\mathbf{s}^H \right] = \mathbf{I}_{K} \right)$. Matrix $\mathbf{W} \in \mathbb{C}^{N \times K}$ is the linear precoding matrix to be designed. As mentioned previously, each DVB-S2X frame contains information intended to multiple users in order to attain a large channel coding gain. In this context, every UT user with index $i=1,\ldots,N_{u}$ at the $k$-th beam shall detect the same information $[\mathbf{s}] _{k}$, leading to the so-called multigroup multicast transmission{\color{blue}, which has already been studied for the general wireless systems in \cite{karipidis2008quality}}.

The system sum-rate is defined as $\mathcal{SR} = \sum_{k = 1}^K \min_{i = 1, \ldots , N_u} \quad \log_2 \left(1 + \text{SINR}_k^{[i]} \right),$ where $\text{SINR}_k^{[i]}$ is the signal-to-noise-plus-interference ratio (SINR) of the $i$-th user at the $k$-th beam and is defined as
\begin{equation}\label{sinr}
\text{SINR}_k^{[i]}= \frac{|\mathbf{h}_k^{[i],H}\mathbf{w}_k|^2}{\sum_{j\neq k}|\mathbf{h}_k^{[i],H}\mathbf{w}_j|^2 + 1},
\end{equation}
where $\mathbf{h}_k^{[i],H}$ and $\mathbf{w}_k$ are the $k$-th row and $k$-th column of $\mathbf{H}^{[i]}$ and $\mathbf{W}$, respectively. Note that since we are considering a multicast transmission, the achievable data rate at each beam is determined by the data rate that the UT with the lowest SINR can achieve, as the selected MODCOD for transmission should be decodable by all UTs in the frame.

As a matter of fact, the system designer should find a solution to the following optimization problem:
\begin{equation}
\begin{aligned}
& \mathcal{P}_1: \quad  \underset{\mathbf{W} }{\text{maximize}} \quad  \mathcal{SR} \\
& \text{subject to}\\
& \left[\mathbf{W}\mathbf{W}^H \right]_{nn} \leq  P \quad n = 1 , \ldots , N. \\
\end{aligned}
\end{equation}
The optimization problem $\mathcal{P}_1$ is large-scale and non-convex (the objective function is non-convex). Note that in $\mathcal{P}_1$ a matrix of around 10,000 complex elements shall be optimized over hundreds of per-feed power constraints. { \color{blue} The work in \cite{christopoulos2014weighted} considers the optimization of $\mathcal{P}_1$ via a semi-definite relaxation procedure, which is adequate from small to medium coverage areas. In case a notably larger number of beams and/or users are targeted, current non-convex optimization alternatives might fail due to the immense computational complexity; thus, opening potential avenues for future research.}

A promising precoding alternative considering the performance-computational complexity trade-off is the 'UpConst Multicast MMSE' \cite{Taricco2014,Vazquez2016}, which can be written as $\mathbf{W}_{\text{MMSE}} = \beta_{\text{MMSE}}\left(\widehat{\mathbf{H}}^H\widehat{\mathbf{H}} + \frac{1}{P} \mathbf{I}_N \right)^{-1}\widehat{\mathbf{H}}^H,$ where $\beta_{\text{MMSE}}$ controls the transmit power to fulfill the per-feed power constraints and $\widehat{\mathbf{H}} = \frac{1}{N_u} \sum_{i = 1}^{N_u} \mathbf{H}^{[i]}.$ In other words, this design consists of minimum-mean-squared error (MMSE) precoding over the average channel matrix of all users simultaneously served at each beam. The channel elements in $\mathbf{H}^{[i]}$ are reported by each UT in the return link. Section III comments on the estimation of the UT’s channel. In a practical system the channel state information is usually quantized and contains residual errors, affecting the expected gains of the precoding techniques, when compared to the theoretical cases in which the CSIT is perfectly known. Fortunately, FSSs experience low satellite channel variability, and due to that, the existing studies report a performance improvement via satellite precoding. 

A comprehensive study of linear precoding techniques for the general multigroup multicast communication model can be found in \cite{Silva2009}. Fig. \ref{exam} shows the beam data rate and the computational time of both 'upconst' multicast minimum mean square error (UpConst Multicast MMSE) and the block singular value decomposition (block-SVD) technique presented in \cite{Vazquez2016}. For obtaining the results, we consider a beampattern with 245 beams and a maximum per-feed power constraint of 55 W. Both the average central process unit (CPU) time and the average beam capacity, $SR/K$, have been obtained over 100 Monte Carlo runs. 

\begin{figure}[h!]
	\centering
    \includegraphics[scale = 0.5]{images/sigmag}
    \centering
		\caption{Average beam data rate and average CPU elapsed time of two precoding techniques, MMSE and block-SVD.}
      \label{exam}
\end{figure}

Clearly, the larger $N_u$, the lower are the attainable rates obtained by both block-SVD and UpConst Multicast MMSE. In all cases, Block-SVD leads to larger data rates compared to the UpConst Multicast MMSE. Nevertheless, the computational complexity of UpConst Multicast MMSE is much lower than Block-SVD and does not grow notably when the number of $N_u$ users per frame increases. On the contrary, block-SVD requires more computational time to compute the precoding matrix as the number of UT grows.

However, despite its low computational complexity,  UpConst Multicast MMSE still presents implementation challenges when serving large coverage areas (i.e., the computation of the matrix inverse becomes a computationally demanding operation as $K$ grows). Consequently, the study of alternative precoding designs is of extraordinary interest for both academia and industry. Concretely, it shall be explored precoding techniques that require a limited number of operations, when computing its precoding matrices, while they provide large data rates.

It is important to remark that the scheduling process plays a key role to obtain relevant sum-rate values; as it is crucial to select the most convenient users to be served in each satellite frame. As reported in \cite{Vazquez2016}, this scheduling process could just simply consider the geographical position of the UTs. In this way, information from UTs that are geographically close can be embedded into the same frame in order to yield efficient data rates. In any case, an open problem to be tackled is the characterization of the scheduling effect on the overall architecture, bearing in mind the queue's stability and the UT's targeted data rates.

Whenever the high layers are considered, the precoding design should be able to guarantee certain QoS to the UTs. In contrast to cellular systems, satellite operators offer their clients service level agreements (SLA) that involve a minimum data rate over a certain percentage of the channel access attempts. In this case, the fulfillment of the SLA contracts by precoding is done by optimizing the following problem:
\begin{equation*}
\begin{aligned}
& \mathcal{P}_2: \quad  \underset{\mathbf{W} }{\text{minimize}} \quad  \left||\mathbf{W} \right||^2 \\
& \text{subject to}\\
& \left[\mathbf{W}\mathbf{W}^H \right]_{nn} \leq  P \quad n = 1 , \ldots , N, \\
& \text{SINR}_k^{[i]} > \gamma_k \quad k = 1, \ldots , K \quad i = 1, \ldots , N_u.
\end{aligned}
\end{equation*}
The optimization problem $\mathcal{P}_2$ is a non-convex quadratically constrained quadratic problem (QCQP){\color{blue}, which limits its applicability in large-scale coverage areas. This problem can be tackled via semi-definite relaxation (SDR) approximation methods such as the one in \cite{Karipidis2008}}. Bearing this in mind, efficient parallel implementation of the non-convex QCQP optimization tools can be a good alternative for solving $\mathcal{P}_2$ in real multibeam satellite systems. {\color{blue} This is the case for the work done in \cite{Vazquez2017}, which promotes the use of the consensus alternate direction of multipliers method of \cite{Huang2016} to solve the non-convex QCQP $\mathcal{P}_2$.}


